Cryo-Electron Microscopy Image Analysis Using Multi-Frequency Vector Diffusion Maps

Cryo-electron microscopy (EM) single particle reconstruction is an entirely general technique for 3D structure determination of macromolecular complexes. However, because the images are taken at low electron dose, it is extremely hard to visualize the individual particle with low contrast and high noise level. In this paper, we propose a novel approach called multi-frequency vector diffusion maps (MFVDM) to improve the efficiency and accuracy of cryo-EM 2D image classification and denoising. This framework incorporates different irreducible representations of the estimated alignment between similar images. In addition, we propose a graph filtering scheme to denoise the images using the eigenvalues and eigenvectors of the MFVDM matrices. Through both simulated and publicly available real data, we demonstrate that our proposed method is efficient and robust to noise compared with the state-of-the-art cryo-EM 2D class averaging and image restoration algorithms.

==> textfiles/Parameters.tex <==
\section{Details of MFVDM Parameter Choice}
\label{sec:param}

In this section We provide detailed discussions about: (1)MFVDM preprocessing, (2)the choice of parameters for MFVDM nearest neighbor search and denoising. Due to limited space, most of them are only slightly mentioned in our main paper. Specifically, we illustrate our strategy of hyperparameter settings of MFVDM, by presenting experimental results. 

\vspace{0.1cm}
\noindent\textbf{Preprocessing: }We divide the preprocessing into three steps: (1)standardization, (2)whitening, and (3)phase flipping. Standardization is to normalize the noise on each raw image, i.e, make noise have zero mean and variance one. We whiten our data since the real data noise statistics is usually colored. Then phase flipping is used to compensate the influence of CTFs on the phase of Fourier domain.

\vspace{0.1cm}
\noindent\textbf{Nearest Neighbor Search: }
In our experiments, based on the initial classification results in Sec~\ref{sec:init}, we identify 50 nearest neighbors for each node and build the graph. The nearest neighbor search uses the maximum frequency $\tilde{k} = 10$ and the truncation $m = 50$ for the MFVDM embedding. The strategy of such parameter setting is to seek a balance between bias and variance. Too many MFVDM eignevectors will introduce spurious information. Not enough eigenvectors incurs approximation error. Empirically we find the nearest neighbor search result is not very sensitive to the choice of $\tilde{k}$ and $m$. As long as they are in a reasonable range, the results are similar.  

\vspace{0.1cm}
\noindent\textbf{Rotational Alignment: }
For rotational alignment, MFVDM uses FFT to estimate the in-plane rotation between nearest neighbor pairs. In our experiments we zero-pad and set the point of FFT to be 1024, which is not only computationally efficient, but also large enough to get an accurate estimation. A smaller point FFT could increase the approximation error.

\begin{figure*}[t!]
\centering
\setlength\tabcolsep{1.0pt}
\renewcommand{\arraystretch}{0.6}
\begin{tabular}{p{0.01\textwidth}<{\centering} p{0.1305\textwidth}<{\centering}
p{0.130\textwidth}<{\centering}
p{0.130\textwidth}<{\centering} p{0.130\textwidth}<{\centering} p{0.130\textwidth}<{\centering} p{0.130\textwidth}<{\centering} p{0.130\textwidth}<{\centering} p{0.038\textwidth}<{\centering}} 
&\textbf{\scriptsize{Noisy}} &\textbf{\scriptsize{Clean}}
&\textbf{\scriptsize{MFVDM(1)}} &\textbf{\scriptsize{MFVDM(2)}} &\textbf{\scriptsize{MFVDM(3)}} &\textbf{\scriptsize{MFVDM(4)}} &\textbf{\scriptsize{MFVDM(5)}} & \\ 

\raisebox{0.425\height}{\rotatebox{90}{\textbf{\scriptsize{SNR = 0.05}}}}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_filter/noisynoisy_CTF_0_05_ncb.png}
&\includegraphics[width = 0.130\textwidth]{figures/clean_nocolorbar.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_filter/eVDM_filter_1_0_05.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_filter/eVDM_filter_2_0_05.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_filter/eVDM_filter_6_0_05.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_filter/eVDM_filter_5_0_05.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_filter/eVDM_filter_4_0_05.png}
&\includegraphics[width = 0.038\textwidth]{figures/colorbar_new.png}\\ 

\raisebox{0.425\height}{\rotatebox{90}{\textbf{\scriptsize{SNR = 0.02}}}}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_filter/noisynoisy_CTF_0_02_ncb.png}
&\includegraphics[width = 0.130\textwidth]{figures/clean_nocolorbar.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_filter/eVDM_filter_1_0_02.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_filter/eVDM_filter_2_0_02.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_filter/eVDM_filter_6_0_02.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_filter/eVDM_filter_5_0_02.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_filter/eVDM_filter_4_0_02.png}
&\includegraphics[width = 0.038\textwidth]{figures/colorbar_new.png}\\ 

\raisebox{0.425\height}{\rotatebox{90}{\textbf{\scriptsize{SNR = 0.01}}}}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_filter/noisynoisy_CTF_0_01_ncb.png}
&\includegraphics[width = 0.130\textwidth]{figures/clean_nocolorbar.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_filter/eVDM_filter_1_0_01.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_filter/eVDM_filter_2_0_01.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_filter/eVDM_filter_6_0_01.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_filter/eVDM_filter_5_0_01.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_filter/eVDM_filter_4_0_01.png}
&\includegraphics[width = 0.038\textwidth]{figures/colorbar_new.png}\\ 
\end{tabular}
\caption{Image samples of denoising results on 70S ribosome, by MFVDM with different type of filters, from \textit{left} to \textit{right}: Noisy projection images, clean projection images, denoised results by MFVDM(1), MFVDM(2), MFVDM(3), MFVDM(4), MFVDM(5). Rows show different noise levels $\text{SNR} = 0.05,0.02,0.01$.}
\label{fig:eVDM_filter}
\end{figure*}

\renewcommand{\arraystretch}{0.8}
\setlength{\textfloatsep}{0.2cm}
\begin{table}[t!]
\caption{Average MSE, PSNR and SSIM of denoised images on 70S ribosome, by different MFVDM filters.}
\centering
\begin{tabular}{p{0.04\textwidth}<{\centering}| p{0.05\textwidth}<{\centering}| p{0.09\textwidth}<{\centering} p{0.09\textwidth}<{\centering} p{0.09\textwidth}<{\centering} p{0.09\textwidth}<{\centering}  p{0.09\textwidth}<{\centering}} \toprule
\multicolumn{2}{c|}{\multirow{2}{*}{\raisebox{-0.2pt}{SNR}}} & \multicolumn{5}{c}{Different filters for MFVDM} \\ %\cmidrule{3-7}
\multicolumn{2}{c|}{}  &MFVDM(1) &MFVDM(2) &MFVDM(3) &MFVDM(4) &MFVDM(5) 
\\ \midrule
\multirow{3}{*}{0.05} &MSE &0.0207 &0.0177 &0.0208 &\textbf{0.0104} &0.0139\\
                  &PSNR &46.9 &47.7 &46.9 &\textbf{49.9}  &48.6 \\
                  &SSIM &0.963 &0.966 &0.963 &\textbf{0.974} &0.967 \\ \midrule
\multirow{3}{*}{0.02} &MSE &0.0241 &\textbf{0.0223} &0.0242 &0.0223 &0.0242 \\
                  &PSNR &46.4 &\textbf{46.7} &46.4 &46.7 &46.3 \\
                  &SSIM &0.957 &\textbf{0.959} &0.957 &0.958 &0.957 \\ \midrule
\multirow{3}{*}{0.01} &MSE &0.0419 &\textbf{0.0383} &0.0411 &0.0638 &0.115 \\
                  &PSNR &44.1 &\textbf{44.6} &44.2 &42.6  &40.0 \\
                  &SSIM &0.930 &\textbf{0.932} &0.931 &0.908 &0.854 \\ 
\bottomrule
\end{tabular}
\label{tab:eVDM_filter_mse,ssim,psnr}
\end{table}

\vspace{0.1cm}
\noindent\textbf{Denoising: }We do denoising by applying an appropriated filter (denote as $h(\lambda)$, where $\lambda$ is the eigenvalue of the operator $S_k$, please refer to eq.(3) in our main paper) on the Fourier-Bessel coefficients of the raw images, and we truncate the filter with its top $m$ eigenvectors to further reduce noise. Apparently the denoised results could be sensitive to the choice of filters and truncation $m$. Here we introduce five filters that may be useful:
\begin{itemize}
    \item \textbf{MFVDM(1): }$h(\lambda) = \lambda$, and we truncate it with the top $m = 50$ eigenvalues.
    \item \textbf{MFVDM(2): }$h(\lambda) = 2\lambda - \lambda^2$, also we truncate it with the top $m = 50$ eigenvalues. \textbf{This is the filter we used in our main paper}. It can be thought as we first apply MFVDM(1), and then we apply MFVDM(1) on the residual part, sum these two parts together we get MFVDM(2) as $h(\lambda) = \lambda + \lambda(1-\lambda) = 2\lambda - \lambda^2$.
    \item \textbf{MFVDM(3): }$h(\lambda) = \lambda^3 - 3\lambda^2 + 3\lambda$, also we truncate with the top $m = 50$ eigenvalues. This filter can be thought as we first apply MFVDM(2), and then we apply MFVDM(1) on the residual part, sum these two parts together we get MFVDM(3).
    \item \textbf{MFVDM(4): }$h(\lambda) = \lambda$ without truncation.
    \item \textbf{MFVDM(5): }$h(\lambda) = 2\lambda - \lambda^2$ without truncation.
\end{itemize}

To compare these filters, in Fig.~\ref{fig:eVDM_filter} we present the denoising results on 70S ribosome data, also in Tab.~\ref{tab:eVDM_filter_mse,ssim,psnr} we show their corresponding MSE, PSNR and SSIM. We observe that at high SNR case as $\text{SNR} = 0.05$, applying the average operator $S_k$ directly (i.e., eVDM(4)) could be better than truncating with top eigenvalues, since clean signal is preserved by keeping all the eigenvectors and truncation could lost such signal. When noise level is increasing as $\text{SNR} = 0.01$, truncation becomes necessary, since the eigenvectors corresponding to the small eigenvalues are easily perturbed by noise. Otherwise the denoising results are as blurry as shown in the bottom right corner of Fig.~\ref{fig:eVDM_filter} as eVDM(4) and eVDM(5). Therefore, whether doing truncation or not should depend on a trade-off between noisy and clean signal. Another observation is when doing truncation, using $h(\lambda) = 2\lambda - \lambda^2$ could improve the denoising. 

To further explore the effects of truncation, in Fig.~\ref{tab:eVDM_trun_mse,ssim,psnr} and Tab.~\ref{tab:eVDM_trun_mse,ssim,psnr} we show the denoising results on 70S ribosome and the corresponding MSE, PSNR, SSIM by different number of truncation $m$. Here the filter $h(\lambda) = 2\lambda - \lambda^2$ is used and we varies $m$ from $m = 10$ to $m = 125$, where $m = 50$ is the choice in our main paper. It can be seen that at high SNR cases as $\text{SNR} = 0.05, 0.02$, a larger truncation $m$ could improve the denoising, since more information of the clean signal is preserved. While at $\text{SNR} = 0.01$, the results from a large $m$ as $m = 100, 125$ are noisy, since we have included more eigenvectors that has been perturbed by noise. Again, this emphasizes the choice of $m$ is a trade-off between noise and clean signal. 

\begin{figure*}[t!]
\centering
\setlength\tabcolsep{1.0pt}
\renewcommand{\arraystretch}{0.6}
\begin{tabular}{p{0.01\textwidth}<{\centering} p{0.1305\textwidth}<{\centering} p{0.130\textwidth}<{\centering} p{0.130\textwidth}<{\centering} p{0.130\textwidth}<{\centering} p{0.130\textwidth}<{\centering} p{0.130\textwidth}<{\centering} p{0.130\textwidth}<{\centering} p{0.038\textwidth}<{\centering}} 
&\textbf{\scriptsize{Clean}} &\scriptsize{$\bm{m = 10}$} &\scriptsize{$\bm{m = 25}$} &\scriptsize{$\bm{m = 50}$} &\scriptsize{$\bm{m = 75}$} &\scriptsize{$\bm{m = 100}$} &\scriptsize{$\bm{m = 125}$} & \\ 

\raisebox{0.425\height}{\rotatebox{90}{\textbf{\scriptsize{SNR = 0.05}}}}
&\includegraphics[width = 0.130\textwidth]{figures/clean_nocolorbar.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_trun/eVDM_trun_10_0_05.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_trun/eVDM_trun_25_0_05.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_trun/eVDM_trun_50_0_05.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_trun/eVDM_trun_75_0_05.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_trun/eVDM_trun_100_0_05.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_trun/eVDM_trun_125_0_05.png}
&\includegraphics[width = 0.038\textwidth]{figures/colorbar_new.png}\\ 

\raisebox{0.425\height}{\rotatebox{90}{\textbf{\scriptsize{SNR = 0.02}}}}
&\includegraphics[width = 0.130\textwidth]{figures/clean_nocolorbar.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_trun/eVDM_trun_10_0_02.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_trun/eVDM_trun_25_0_02.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_trun/eVDM_trun_50_0_02.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_trun/eVDM_trun_75_0_02.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_trun/eVDM_trun_100_0_02.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_trun/eVDM_trun_125_0_02.png}
&\includegraphics[width = 0.038\textwidth]{figures/colorbar_new.png}\\ 

\raisebox{0.425\height}{\rotatebox{90}{\textbf{\scriptsize{SNR = 0.01}}}}
&\includegraphics[width = 0.130\textwidth]{figures/clean_nocolorbar.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_trun/eVDM_trun_10_0_01.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_trun/eVDM_trun_25_0_01.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_trun/eVDM_trun_50_0_01.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_trun/eVDM_trun_75_0_01.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_trun/eVDM_trun_100_0_01.png}
&\includegraphics[width = 0.130\textwidth]{figures/eVDM_trun/eVDM_trun_125_0_01.png}
&\includegraphics[width = 0.038\textwidth]{figures/colorbar_new.png}\\ 
\end{tabular}
\caption{Image samples of denoising results on 70S ribosome, by MFVDM with diffrent number of truncation $m$, from \textit{left} to \textit{right}: clean projection images, denoised results by MFVDM with $m = 10,25,50,75,100,125$. Rows show different noise levels $\text{SNR} = 0.05,0.02,0.01$.}
\label{fig:eVDM_truncation}
\end{figure*}

\renewcommand{\arraystretch}{0.8}
\setlength{\textfloatsep}{0.2cm}
\begin{table}[t!]
\caption{Average MSE, PSNR and SSIM of denoised images on 70S ribosome, by different truncation $m$.}
\centering
\begin{tabular}{p{0.04\textwidth}<{\centering}| p{0.05\textwidth}<{\centering}| p{0.08\textwidth}<{\centering} p{0.08\textwidth}<{\centering} p{0.08\textwidth}<{\centering} p{0.08\textwidth}<{\centering} p{0.08\textwidth}<{\centering} p{0.08\textwidth}<{\centering}} \toprule
\multicolumn{2}{c|}{\multirow{2}{*}{\raisebox{-3pt}{SNR}}} & \multicolumn{6}{c}{Different truncation $m$ for MFVDM} \\ %\cmidrule{3-7}
\multicolumn{2}{c|}{}  &$m = 10$ &$m = 25$ &$m = 50$ &$m = 75$ &$m = 100$ &$m = 125$
\\ \midrule
\multirow{3}{*}{0.05} &MSE &0.0542 &0.0384 &0.0177 &0.0174 &0.0163 &\textbf{0.0157}\\
                  &PSNR &42.7 &44.2 &46.9 &47.7 &47.9 &\textbf{48.1} \\
                  &SSIM &0.921 &0.943 &0.963 &0.965 &0.967 &\textbf{0.969}\\ \midrule
\multirow{3}{*}{0.02} &MSE &0.0554 &0.0397 &0.0223 &0.0221 &0.0215 &\textbf{0.0207} \\
                  &PSNR &42.7 &44.8 &46.7 &46.9 &47.0 &\textbf{47.1} \\
                  &SSIM &0.919 &0.939  &0.959 &0.959 &0.960 &\textbf{0.961} \\ \midrule
\multirow{3}{*}{0.01} &MSE &0.0624 &0.0523 &\textbf{0.0383} &0.0459 &0.0468 &0.483 \\
                  &PSNR &42.3 &43.2 &\textbf{44.6} &44.1 &43.9 &43.8 \\
                  &SSIM &0.911 &0.924 &\textbf{0.932} &0.931 &0.929 &0.927 \\ 
\bottomrule
\end{tabular}
\label{tab:eVDM_trun_mse,ssim,psnr}
\end{table}





